In Search of Socio-Technical Congruence: A Large-Scale Longitudinal Study

We report on a large-scale empirical study investigating the relevance of socio-technical congruence over key basic software quality metrics, namely, bugs and churn. In particular, we explore whether alignment or misalignment of social communication structures and technical dependencies in large software projects influences software quality. To this end, we have defined a quantitative and operational notion of socio-technical congruence, which we call socio-technical motif congruence (STMC). STMC is a measure of the degree to which developers working on the same file or on two related files, need to communicate. As socio-technical congruence is a complex and multi-faceted phenomenon, the interpretability of the results is one of our main concerns, so we have employed a careful mixed-methods statistical analysis. In particular, we provide analyses with similar techniques as employed by seminal work in the field to ensure comparability of our results with the existing body of work. The major result of our study, based on an analysis of 25 large open-source projects, is that STMC is not related to project quality measures -- software bugs and churn -- in any temporal scenario. That is, we find no statistical relationship between the alignment of developer tasks and developer communications on the one hand, and project outcomes on the other hand. We conclude that, wherefore congruence does matter as literature shows, then its measurable effect lies elsewhere.

==> tab/cassandra_overview.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Fri Jun 19 19:47:59 2020
  \hline
\# Devs. & 1.0 & 5.7 & 4.0 & 55.0 & 6.0 \\ 
  Avg.~Essential[l] & 0.0 & 0.8 & 0.7 & 3.3 & 0.2 \\ 
  Churn[l] & 0.0 & 4.5 & 4.6 & 10.3 & 1.5 \\ 
  LoC[l] & 1.1 & 6.0 & 6.0 & 10.8 & 1.0 \\ 
  Max.~Nesting[l] & 0.0 & 1.3 & 1.4 & 2.2 & 0.5 \\ 
  \# Motifs & 0.0 & 4.3 & 2.0 & 115.0 & 7.4 \\ 
  \(l_{\text{a}}(|\text{AM}|, |\text{M}|)\) & -0.1 & 0.0 & 0.0 & 0.7 & 0.0 \\ 
  \(r(|\text{AM}|, |\text{M}|)\) & -2.0 & -0.2 & 0.0 & 2.0 & 1.6 \\ 
   \hline


==> tab/hbase_overview.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Fri Jun 19 19:47:59 2020
%  \hline
\# Devs. & 1.0 & 4.0 & 3.0 & 42.0 & 3.9 \tabularnewline 
  Avg.~Essential[l] & 0.0 & 0.8 & 0.7 & 1.9 & 0.2 \tabularnewline 
  Churn[l] & 0.0 & 4.5 & 4.6 & 10.6 & 1.5 \tabularnewline 
  LoC[l] & 3.4 & 6.5 & 6.5 & 11.3 & 1.1 \tabularnewline 
  Max.~Nesting[l] & 0.0 & 1.4 & 1.4 & 2.4 & 0.5 \tabularnewline 
  \# Motifs & 0.0 & 1.7 & 0.0 & 98.0 & 5.8 \tabularnewline 
  \(l_{\text{a}}(|\text{AM}|, |\text{M}|)\) & -0.1 & 0.0 & 0.0 & 0.5 & 0.0 \tabularnewline 
  \(r(|\text{AM}|, |\text{M}|)\) & -2.0 & 1.6 & 2.0 & 2.0 & 0.9 \tabularnewline 


==> tab/tab.tex <==
ActiveMQ & Java & Message Queue & 87 & 2781 & 1471 & 9792 & 6048 & 60241 & 12/05--06/17 & 12/05--06/17 & 12/05--07/17 \\ 
  Ambari & JavaScript & Middleware & 120 & 889 & 301 & 20544 & 19147 & 94700 & 08/11--06/17 & 09/11--06/17 & 11/13--07/17 \tabularnewline 
  Apex & Java, C++ & Middleware & 67 & 71 & 140 & 4736 & 694 & 27553 & 06/12--05/17 & 07/15--06/17 & 08/15--07/17 \tabularnewline 
  Camel & Java & Middleware & 421 & 2145 & 1080 & 28675 & 11384 & 48447 & 03/07--06/17 & 04/07--06/17 & 05/07--07/17 \tabularnewline 
  Cassandra & Java & Distributed DB & 271 & 3045 & 966 & 14028 & 13481 & 13056 & 03/09--06/17 & 03/09--06/17 & 01/09--07/17 \tabularnewline 
  CouchDB & Erlang & Distributed DB & 149 & 1109 & 861 & 10115 & 3255 & 47454 & 03/08--06/17 & 04/08--06/17 & 02/08--07/17 \tabularnewline 
  Geronimo & Java & Framework & 61 & 129 & 518 & 13172 & 781 & 6567 & 08/03--03/13 & 08/03--02/13 & 12/02--12/04 \tabularnewline 
  Groovy & Java, Python & Middleware & 272 & 2599 & 163 & 13277 & 7982 & 3328 & 08/03--06/17 & 09/03--06/17 & 03/15--07/17 \tabularnewline 
  Hadoop & Java, C++ & Distributed DB & 159 & 1976 & 3101 & 15701 & 8087 & 23603 & 05/09--06/17 & 05/09--06/17 & 08/12--05/17 \tabularnewline 
  HBase & Java, C++ & Distributed DB & 208 & 1827 & 944 & 13526 & 18079 & 63981 & 04/07--05/17 & 04/07--06/17 & 02/08--07/17 \tabularnewline 
  Hive & Java, C++ & Middleware & 179 & 2524 & 911 & 10164 & 16782 & 127448 & 09/08--06/17 & 09/08--06/17 & 10/10--07/17 \tabularnewline 
  Ignite & Java, C\# & Middleware & 135 & 293 & 346 & 15559 & 5485 & 23897 & 02/14--06/17 & 11/14--06/17 & 10/14--07/17 \tabularnewline 
  Karaf & Java, JavaScript & Framework & 104 & 797 & 358 & 6055 & 5192 & 12058 & 11/07--06/17 & 04/09--06/17 & 06/10--07/17 \tabularnewline 
  Kudu & C++ & Operative-System & 77 & 155 & 124 & 5959 & 1920 & 5754 & 10/12--07/17 & 08/13--07/17 & 12/15--07/17 \tabularnewline 
  LibCloud & Python & Library & 283 & 389 & 165 & 5232 & 931 & 3658 & 08/09--07/17 & 12/09--07/17 & 05/11--07/17 \tabularnewline 
  Lucene & Java, Python, Perl & Middleware & 108 & 4322 & 2098 & 26245 & 17116 & 293945 & 09/01--06/17 & 10/01--06/17 & 09/01--12/03 \tabularnewline 
  Mahout & Java, C++ & Library & 45 & 670 & 615 & 3867 & 1984 & 44981 & 01/08--05/17 & 01/08--06/17 & 01/08--07/17 \tabularnewline 
  Mesos & C++ & Middleware & 274 & 914 & 511 & 10738 & 7096 & 39655 & 07/13--06/17 & 06/13--06/17 & 07/13--07/17 \tabularnewline 
  REEF & C\#, Java & Middleware & 61 & 79 & 81 & 3005 & 1831 & 15133 & 08/12--07/17 & 09/14--07/17 & 09/14--07/17 \tabularnewline 
  Sentry & Python & Application & 25 & 127 & 126 & 906 & 1787 & 7221 & 12/12--06/17 & 08/13--06/17 & 08/13--07/17 \tabularnewline 
  Spark & Scala & Middleware & 1346 & 4158 & 1580 & 18252 & 16261 & 28333 & 03/10--06/17 & 10/12--06/17 & 06/13--07/17 \tabularnewline 
  Subversion & C & Application & 92 & 156 & 853 & 57692 & 4323 & 36361 & 03/00--06/17 & 03/01--06/17 & 03/00--07/17 \tabularnewline 
  Thrift & C++ & Framework & 203 & 1782 & 270 & 4982 & 4209 & 41053 & 07/06--05/17 & 05/08--06/17 & 10/10--07/17 \tabularnewline 
  TrafficServer & C++ & Application & 240 & 496 & 384 & 9454 & 5086 & 13523 & 10/09--07/17 & 10/09--01/17 & 08/09--07/17 \tabularnewline 
  Wicket & Java & Framework & 82 & 1889 & 740 & 19895 & 6388 & 22612 & 09/04--06/17 & 10/06--06/17 & 09/06--07/17 \tabularnewline 
  Zeppelin & Java & Application & 257 & 773 & 308 & 3094 & 2588 & 48710 & 06/13--06/17 & 03/15--06/17 & 01/15--07/17 \tabularnewline


==> tab/tt_summary.tex <==
  Ambari & $100\pm 0\%$ & $100\pm 2\%$ & $100\pm 0\%$ & Kudu & $100\pm 0\%$ & $100\pm 0\%$ & $100\pm 0\%$ \\ 
  Apex & $92\pm 2\%$ & $92\pm 2\%$ & $83\pm 17\%$ & LibCloud & $86\pm 0\%$ & $89\pm 7\%$ & $88\pm 6\%$ \\ 
  Camel & $100\pm 1\%$ & $100\pm 0\%$ & $100\pm 0\%$ & Lucene & $NA\pm 2\%$ & $NA\pm 1\%$ & $NA\pm 2\%$ \\ 
  Cassandra & $98\pm 0\%$ & $100\pm 2\%$ & $98\pm 2\%$ & Mahout & $95\pm 16\%$ & $92\pm 11\%$ & $96\pm 11\%$ \\ 
  CouchDB & $100\pm 29\%$ & $100\pm 32\%$ & $100\pm 17\%$ & Mesos & $100\pm 4\%$ & $100\pm 0\%$ & $100\pm 0\%$ \\ 
  Geronimo & $100\pm 0\%$ & $100\pm 0\%$ & $100\pm 0\%$ & REEF & $82\pm 21\%$ & $94\pm 8\%$ & $94\pm 8\%$ \\ 
  Groovy & $100\pm 8\%$ & $100\pm 2\%$ & $100\pm 8\%$ & Sentry & $83\pm 10\%$ & $86\pm 10\%$ & $82\pm 3\%$ \\ 
  Hadoop & $100\pm 2\%$ & $100\pm 2\%$ & $100\pm 0\%$ & Spark & $100\pm 13\%$ & $100\pm 6\%$ & $100\pm 6\%$ \\ 
  HBase & $97\pm 2\%$ & $97\pm 2\%$ & $100\pm 0\%$ & Thrift & $91\pm 12\%$ & $90\pm 2\%$ & $95\pm 5\%$ \\ 
  Hive & $98\pm 0\%$ & $98\pm 2\%$ & $95\pm 3\%$ & TrafficServer & $91\pm 7\%$ & $97\pm 3\%$ & $97\pm 5\%$ \\ 
  Ignite & $95\pm 0\%$ & $100\pm 0\%$ & $NA\pm NA\%$ & Wicket & $94\pm 13\%$ & $99\pm 6\%$ & $99\pm 12\%$ \\ 


==> tab/tt_summary2_jira.tex <==
activemq & 83\% & 91\% & 89\% & 97\% & 92\% & 92\% & 89\% & 94\% & 84\% & karaf & 70\% & 68\% & 60\% & 86\% & 94\% & 76\% & 79\% & 94\% & 74\% \\ 
  ambari & 100\% & 100\% & 100\% & 100\% & 98\% & 100\% & 100\% & 100\% & 100\% & kudu & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\ 
  apex & 90\% & 92\% & 92\% & 90\% & 92\% & 92\% & 80\% & 75\% & 92\% & libcloud & 100\% & 100\% & 100\% & 93\% & 100\% & 100\% & 100\% & 100\% & 94\% \\ 
  camel & 99\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & lucene & 94\% & 95\% & 94\% & 99\% & 98\% & 98\% & 96\% & 98\% & 97\% \\ 
  cassandra & 98\% & 98\% & 98\% & 98\% & 100\% & 100\% & 96\% & 98\% & 100\% & mahout & 91\% & 92\% & 76\% & 91\% & 93\% & 83\% & 88\% & 97\% & 85\% \\ 
  couchdb & 53\% & 71\% & 100\% & 62\% & 94\% & 100\% & 72\% & 89\% & 100\% & mesos & 96\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\ 
  geronimo & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & reef & 73\% & 93\% & 92\% & 92\% & 100\% & 94\% & 92\% & 100\% & 94\% \\ 
  groovy & 81\% & 79\% & 88\% & 86\% & 88\% & 88\% & 82\% & 89\% & 88\% & sentry & 77\% & 87\% & 92\% & 79\% & 88\% & 93\% & 87\% & 83\% & 87\% \\ 
  hadoop & 97\% & 98\% & 98\% & 98\% & 98\% & 100\% & 98\% & 98\% & 98\% & spark & 83\% & 84\% & 96\% & 93\% & 94\% & 100\% & 90\% & 94\% & 100\% \\ 
  hbase & 98\% & 98\% & 100\% & 98\% & 100\% & 98\% & 100\% & 100\% & 100\% & thrift & 83\% & 77\% & 89\% & 92\% & 90\% & 92\% & 93\% & 91\% & 96\% \\ 
  hive & 94\% & 94\% & 94\% & 95\% & 97\% & 97\% & 91\% & 94\% & 97\% & trafficserver & 91\% & 93\% & 100\% & 97\% & 97\% & 100\% & 91\% & 97\% & 98\% \\ 
  ignite & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & wicket & 76\% & 90\% & 79\% & 92\% & 97\% & 90\% & 85\% & 97\% & 85\% \\ 


==> tab/tt_summary2_mail_jira.tex <==
activemq & 89\% & 95\% & 90\% & 100\% & 96\% & 100\% & 95\% & 96\% & 91\% & karaf & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% \\ 
  ambari & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & kudu & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\ 
  apex & 90\% & 92\% & 92\% & 90\% & 92\% & 92\% & 80\% & 83\% & 92\% & libcloud & 80\% & 86\% & 100\% & 86\% & 89\% & 100\% & 83\% & 88\% & 100\% \\ 
  camel & 99\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & lucene & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% & NA\% \\ 
  cassandra & 95\% & 98\% & 98\% & 97\% & 100\% & 100\% & 92\% & 98\% & 98\% & mahout & 89\% & 95\% & 70\% & 89\% & 92\% & 83\% & 85\% & 96\% & 85\% \\ 
  couchdb & 83\% & 100\% & 100\% & 100\% & 100\% & 100\% & 86\% & 100\% & 100\% & mesos & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\ 
  geronimo & 100\% & 100\% & NA\% & NA\% & 100\% & NA\% & 100\% & 100\% & NA\% & reef & 88\% & 82\% & 100\% & 90\% & 94\% & 100\% & 91\% & 94\% & 100\% \\ 
  groovy & 79\% & 100\% & 75\% & 86\% & 100\% & 58\% & 71\% & 100\% & 75\% & sentry & 73\% & 83\% & 100\% & 76\% & 86\% & 94\% & 78\% & 82\% & 100\% \\ 
  hadoop & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% & spark & 96\% & 100\% & 92\% & 96\% & 100\% & 96\% & 96\% & 100\% & 96\% \\ 
  hbase & 97\% & 97\% & 93\% & 99\% & 97\% & 99\% & 97\% & 100\% & 97\% & thrift & 86\% & 91\% & 86\% & 100\% & 90\% & 85\% & 95\% & 95\% & 95\% \\ 
  hive & 98\% & 98\% & 93\% & 100\% & 98\% & 94\% & 96\% & 95\% & 94\% & trafficserver & 96\% & 91\% & 96\% & 100\% & 97\% & 100\% & 97\% & 97\% & 100\% \\ 
  ignite & 100\% & 95\% & 100\% & 100\% & 100\% & 100\% & NA\% & NA\% & NA\% & wicket & 80\% & 94\% & 80\% & 90\% & 99\% & 93\% & 86\% & 99\% & 87\% \\ 

